A Gauss-Seidel method for solving multi-leader-multi-follower games

We design a computational approach to find equilibria in a class of Nash games possessing a hierarchical structure. By using tools from mixed-integer optimization and the characterization of variational equilibria in terms of the Karush-Kuhn-Tucker conditions, we propose a mixed-integer game formulation for solving this challenging class of problems. Besides providing an equivalent reformulation, we design a proximal Gauss--Seidel method with global convergence guarantees in case the game enjoys a potential structure. We finally corroborate the numerical performance of the algorithm on a novel instance of the ride-hail market problem.

==> graveyard.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{multipliers}
    \caption{Lagrange multipliers of firm $1$ (colored solid lines) for the constraints in \eqref{eq:cust_demand}, obtained in one of the $50$ random numerical instances. The dashed colored lines denote the upper-bound imposed through \eqref{eq:single-level-reform:ll-constr-4b}.}
    \label{fig:multipliers}
\end{figure}

With this regard, Fig.~\ref{fig:multipliers} illustrates an example of the evolution of the nonnegative Lagrange multipliers associated to firm $1$ in one of the $50$ random instances, which stay always below the upper-bound imposed through \eqref{eq:single-level-reform:ll-constr-4b} with $\mc M^i_\nu$ as in Tab.~\ref{tab:sim_val}.

==> keywords.tex <==
Single-leader-multi-follower games,
Single-level reformulations%
%
%
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "mlmf-via-gs-milp"
%%% End:


==> msc2020.tex <==
TODO%
%
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "mlmf-via-gs-milp"
%%% End:

